Designing Computational Tools for Exploring Causal Relationships in Qualitative Data

Exploring causal relationships for qualitative data analysis in HCI and social science research enables the understanding of user needs and theory building. However, current computational tools primarily characterize and categorize qualitative data; the few systems that analyze causal relationships either inadequately consider context, lack credibility, or produce overly complex outputs. We first conducted a formative study with 15 participants interested in using computational tools for exploring causal relationships in qualitative data to understand their needs and derive design guidelines. Based on these findings, we designed and implemented QualCausal, a system that extracts and illustrates causal relationships through interactive causal network construction and multi-view visualization. A feedback study (n = 15) revealed that participants valued our system for reducing the analytical burden and providing cognitive scaffolding, yet navigated how such systems fit within their established research paradigms, practices, and habits. We discuss broader implications for designing computational tools that support qualitative data analysis.

==> sections/method_discard.tex <==
\section{Methods}
\label{sec:method}

% To understand researchers' perspectives on the role of computational tools in qualitative-data analysis, we conducted two studies: a \textit{formative study} and a \textit{feedback study}.
% The formative study aimed to identify the current challenges researchers face when analyzing qualitative data, how they currently use computational tools, and how such tools could better support their work.
% This study consisted of a need-finding workshop with 15 researchers who had prior experience using computational tools for qualitative-data analysis or who expressed interest in incorporating such tools into their research practices.
Based on the findings of the formative study, we developed design goals for computational systems that support qualitative-data analysis, which guided our implementation of \texttt{QualCausal}.
Next, we conducted a feedback study with \texttt{QualCausal} to identify opportunities for designers to develop and deploy computational methods that can effectively integrate into qualitative-data analysis workflows. 
We used \texttt{QualCausal} to elicit researchers' thoughts and experiences.
We recruited 15 participants for this study, eight of whom had participated in the formative study.


\subsection{Study Procedures}

\subsubsection{Formative Study}

Our formative study consisted of a 2-hour \textbf{workshop} with 15 researchers, facilitated by three members of the research team. 
The workshop was conducted in person in a seminar room equipped with whiteboards and collaborative materials.

We began with a 10-minute session in which participants introduced themselves and shared their research backgrounds, as well as their experience with qualitative-data analysis and computational methods. 
We then provided a 20-minute introduction to key approaches. 
We introduced widely used qualitative-data analysis methods, particularly grounded theory \cite{grounded_theory_larossa_2005}, which was likely new to researchers who primarily conduct content analysis \cite{content_analysis_krippendorff_2018} on qualitative data using computational methods, as well as common computational approaches, such as topic modeling \cite{topic_modeling_rodriguez_2020} and NLP-based causal inference \cite{causal_text_meng_2025, causal_nlp_feuerriegel_2025}, which primarily target researchers whose work involves methods like ethnography and thematic analysis.


After the opening introductions, we divided the participants into four groups of three to four people each. 
We intentionally mixed researchers from different methodological backgrounds to encourage diverse perspectives within each group. 
We posed three discussion questions for the groups to consider: 1) their current knowledge of computational methods for analyzing qualitative data, with those who had used computational tools sharing their experiences and those interested in using such methods discussing what they had heard about or wanted to try; 2) the challenges they face when analyzing qualitative data; and 3) their vision for how intelligent computational tools could support qualitative-data analysis. 
Each question received five minutes of group discussion time, followed by two and a half minutes for each group to share their insights with all participants using post-it notes on the whiteboard.

In the final activity, participants used colored pens and paper to individually sketch their envisioned system for qualitative-data analysis. 
We chose \textit{paper prototyping} to encourage rapid ideation without technical constraints \cite{paper_prototyping_2003}.
The exercise took 15 minutes, followed by two minutes per person to share and discuss their designs. 
We concluded the workshop by providing key takeaways and contact information for those interested in signing up for follow-up studies (i.e., feedback study). 
Figure \ref{fig:study_design} (a) illustrates the workshop procedure.



\subsubsection{Feedback Study}

We conducted a feedback study with 15 researchers, using \texttt{QualCausal} as a backdrop to scaffold broader conversations about the role of computational tools in the space of qualitative research. 
The study involved a 60-minute in-person session with each participant, facilitated by the first author. 

After receiving permission to audio record the sessions, we introduced the participants to our example dataset and explained that the purpose of the session was to use our system to analyze this sample of qualitative data in order to discuss computational tools for qualitative-data analysis more broadly.
We then walked the participants through our system \cite{walkthrough_light_2018} and introduced its main functional modules. 
We sent participants the link to \texttt{QualCausal} and asked them to open it on their laptops and think aloud as they interacted with the system \cite{think_aloud_hertzum_2024}. 
During their hands-on exploration, we provided step-by-step guidance to help them apply the system to conceptualize the given data, collaborate with the system to semi-automatically build the causal network, and navigate the generated network using visual panels.
When participants were uncertain about how to proceed, we offered gentle reminders.

The following interview began by asking participants about their experiences with our sample data and system. 
We asked what they achieved using our system on the sample data, how they interacted with the system to achieve their analytical goals, how they felt the system was helpful, and where they thought the system potentially made things worse or created challenges. 
The interview then broadened to explore more general scenarios, asking about what computational models they found beneficial or helpful, and what computational approaches they felt were not appropriate to incorporate, or presented risks and challenges in qualitative inquiry.
This process is summarized in Figure \ref{fig:study_design} (b).

\paragraph{\textcolor{darkred}{\textbf{Sample Dataset.}}}
To foster deeper engagement and discussion, we used a sample human-chatbot dataset about mental-health stigma \cite{sample_data_meng_2025} as our example case, which we determined was suitable for using computational methods for qualitative-data analysis and causal discovery after consulting with computational social scientists on our team.
The dataset contained 20 responses from participants answering the question "\textit{If you were in the process of selecting a tenant for your home, would you feel comfortable entrusting it to someone like Avery?}" 
A sample response was "\textit{Not at all. Unforeseen events and not knowing how the person will react on other days. Avery might have mood swings and cannot control them.}" 
Our research scenario focused on exploring how stigma forms, specifically investigating what causes stigma and the underlying mechanisms. 


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/figure_study_design.pdf}
    \caption{Processes of formative study and feedback study. (a) The formative study was a 2-hour workshop consisting of an introduction (10 minutes), introduction of common methods (20 minutes), group discussions on three questions (15 minutes each), and a co-design activity for computational tools (45 minutes). (b) The feedback study was a 1-hour session consisting of an introduction and system tutorial (10 minutes), followed by two hands-on evaluation sessions (15 minutes each) with \texttt{QualCausal}, and concluding with an experience discussion (15 minutes).}
    \label{fig:study_design}
\end{figure}




\subsection{Participants}

We recruited participants for the formative study through a computational social science summer institute held at a local university.
This week-long program brought together graduate students, postdoctoral researchers, and early-career faculty interested in computational tools in the social sciences.
One of our research team members served as a guest speaker at the institute, and another served as an organizer, which facilitated our recruitment efforts.
We recruited feedback study participants through multiple channels: formative study participants who expressed interest in continuing to the feedback study; additional researchers recruited through our research team's professional networks, as four team members had extensive experience using computational methods for qualitative-data analysis; and participants recruited through Telegram group channels.
Both studies received approval from our institutional ethics review committee.

Four early-stage faculty members, two industry researchers, and nine Ph.D. students participated in the formative study workshop (Table \ref{tab:participants}). 
Five faculty members, four industry researchers, and six PhD students participated in the feedback study (Table \ref{tab:participants}). 
Participants came from diverse research fields and varied in their experience with qualitative-data analysis. 
For the feedback study, we balanced recruitment between researchers who had prior experience using computational tools for qualitative-data analysis ($n=7$) and those who were interested in using such methods but had limited experience ($n=8$). 
We compensated Ph.D. students with approximately US\$11 and faculty/industry researchers with approximately US\$22 via local currency for the one-hour session.



\begin{table}
  \centering
  \small
  \caption{Participant demographics and study participation. F\# denotes faculty members, I\# denotes industry researchers, and P\# denotes Ph.D. students.}
    \begin{tabularx}{\textwidth}{>{\centering\arraybackslash}p{0.10\textwidth} >{\centering\arraybackslash}p{0.15\textwidth} >{\raggedright\arraybackslash}p{0.24\textwidth} >{\centering\arraybackslash}p{0.20\textwidth} >{\centering\arraybackslash}p{0.08\textwidth} >{\centering\arraybackslash}p{0.10\textwidth}}
    \toprule
    \multirow{2}[1]{*}{\textbf{Participant ID}} & 
    \multirow{2}[1]{*}{\textbf{Age}} & 
    \multirow{2}[1]{*}{\textbf{Research Field}} & 
    \multirow{2}[1]{*}{\begin{minipage}[c]{0.18\textwidth}\centering\textbf{Qualitative-data Analysis Experience}\end{minipage}} & 
    \multicolumn{2}{c}{\textbf{Study Participation}} \\
    \cmidrule(lr){5-6}
    & & & & 
    \textbf{Formative} & 
    \textbf{Feedback} \\
    \midrule
    F1 (M) & 25-34 years old & Political Science, Computer Science, Public Policy & 1-2 years & \checkmark & \checkmark/yes \\
    F2 (M) & 35-44 years old & Sociology, Political Science, Communication Studies & 1-2 years & \checkmark & \checkmark/yes \\
    F3 (M) & 25-34 years old & Sociology, Demography & 1-2 years & \checkmark & \checkmark/no \\
    F4 (M) & 35-44 years old & Information Science/HCI & 6-10 years &  & \checkmark/yes \\
    F5 (F) & 35-44 years old & Social Work & More than 10 years &  & \checkmark/no \\
    F6 (M) & 35-44 years old & Linguistics & 3-5 years & \checkmark &  \\
    I1 (F) & 35-44 years old & Education & Less than 1 year & \checkmark &  \\
    I2 (F) & 35-44 years old & Psychology, Education & 3-5 years &  & \checkmark/no \\
    I3 (F) & 25-34 years old & Computer Science & 6-10 years & \checkmark & \checkmark/no \\
    I4 (F) & 35-44 years old & Communication Studies, Public Health & 6-10 years &  & \checkmark/no \\
    I5 (F) & 25-34 years old & Information Science/HCI & 6-10 years &  & \checkmark/yes \\
    P1 (F) & 18-24 years old & Communication Studies & 6-10 years &  & \checkmark/no \\
    P2 (M) & 25-34 years old & Business/Management, Economics & Less than 1 year & \checkmark &  \\
    P3 (M) & 25-34 years old & Communication Studies & Less than 1 year & \checkmark &  \\
    P4 (F) & 25-34 years old & Sociology, Communication Studies & 6-10 years &  & \checkmark/no \\
    P5 (M) & 25-34 years old & Psychology & 3-5 years & \checkmark &  \\
    P6 (M) & 25-34 years old & Political Science, Public Administration & 1-2 years & \checkmark &  \\
    P7 (F) & 25-34 years old & Information Science/HCI & 1-2 years & \checkmark &  \\
    P8 (F) & 25-34 years old & Communication Studies & 3-5 years & \checkmark & \checkmark/yes \\
    P9 (M) & 25-34 years old & Communication Studies & 3-5 years & \checkmark & \checkmark/yes \\
    P10 (M) & 25-34 years old & Sociology & 1-2 years & \checkmark & \checkmark/yes \\
    P11 (M) & 25-34 years old & Communication Studies & Less than 1 year & \checkmark &  \\
    P12 (F) & 25-34 years old & Communication Studies & 3-5 years &  & \checkmark/no \\
    \bottomrule
    \end{tabularx}%
    \vspace{0.5em}
    \raggedright
    \small
    \textit{Note:} In the \textit{Feedback} column, "yes/no" indicates whether participants have previous experience using computational methods for qualitative-data analysis.

  \label{tab:participants}%
\end{table}


\subsection{Data Analysis}


We video-recorded the workshop for the formative study and used Zoom to automatically transcribe it. 
For the feedback study, we audio-recorded and transcribed the in-person sessions using Microsoft Word. 
We performed thematic analysis \cite{thematic_analysis_braun_2006} on the transcripts from both studies. 
The first author open-coded the transcripts to identify patterns in the dataset. 
Then, the full research team discussed and identified themes. 
The final codebook contained three themes and 22 codes for the formative study and 16 themes and 59 codes for the feedback study. 
We also conducted content analysis \cite{sketch_analysis_buxton_2007} on the participants' design sketches from the formative study.
These findings are discussed in Sections \ref{sec:formative} and \ref{sec:feedback}, respectively.

